A survey of advances in epistemic logic program solvers

Recent research in extensions of Answer Set Programming has included a renewed interest in the language of Epistemic Specifications, which adds modal operators K ("known") and M ("may be true") to provide for more powerful introspective reasoning and enhanced capability, particularly when reasoning with incomplete information. An epistemic logic program is a set of rules in this language. Infused with the research has been the desire for an efficient solver to enable the practical use of such programs for problem solving. In this paper, we report on the current state of development of epistemic logic program solvers.

==> ELPSolverSurvey_Motivation.tex <==
%-------------------------%
% ELPsWVCs_Motivation.tex %
%-------------------------%

\section{Motivation for World View Constraints}\label{MotivSec}

It is well known (see, for example, Proposition 2 in
\cite{LifschitzTangTurner99a}) that constraints (headless rules) in an ASP
program have the net effect of, at most, ruling out certain answer sets from
the program (modulo its constraints). To illustrate, consider the following ASP
program:

\indent $p \ASPor q.$\\
\indent $p \leftarrow q.$

\noindent
which has one answer set $\{p\}$. If we add the constraint

\indent $\leftarrow p, \ASPnot q.$

\noindent
the resulting program has no answer set since $\{p\}$ violates this constraint.

With Epistemic Specifications, constraints can have an additive or subtractive
effect on belief sets or entire world views. Consider, for example, the
following ELP:

\indent $p \ASPor q.$\\
\indent $r \leftarrow \M\ q.$

\noindent
with world view $\{\{p,r\},\{q,r\}\}$. If we add the constraint

\indent $\leftarrow q.$

\noindent
the resulting program has world view $\{\{p\}\}$. Let's look at another
example:

\indent $p \ASPor q.$\\
\indent $r \leftarrow \M\ p.$\\
\indent $s \ASPor t \leftarrow \K\ p.$

\noindent
This program has a single world view, $\{\{p,r\},\{q,r\}\}$. If we add the
constraint

\indent $\leftarrow \M\ p,~\M\ q.$

\noindent
the resulting program has two world views per ES2016:
$\{\{p,r,s\},\{p,r,t\}\}$ and $\{\{q\}\}$.

The previous examples illustrate potential differences in the effect of
constraints on an ELP compared to an ASP program. The last may also show how
constraints can be a possible source of confusion with respect to world
views.\footnote{Should the program even have a world view? Under the earlier
ES1994 semantics, it does not!}
Consider another example:

\indent $p \ASPor q.$\\
\indent $\leftarrow \leftASPnot \K\ p.$

\noindent
Under ES2016 semantics, its world view is $\{\{p\}\}$; however, under the
original semantics \cite{Gelfond91a}, the program has no world view. This
raises the question:

\emph{Which result is more intuitive?}

\noindent
If the intent of the constraint is to rule out \emph{world views} that do not
contain $p$ in every belief set, then the latter (from the original semantics)
would seem correct. Under the later semantics, the net effect of the constraint
is to eliminate \emph{belief sets} that would otherwise result in a world view
that violates the constraint.

For ES2014 semantics, it was shown in \cite{KahlWatsonBalaiGelfondZhang15a}
that, in general, to eliminate \emph{world views} that do not contain $p$ in
every belief set (and not simply eliminate belief sets from a world view that
would otherwise not meet this requirement), two constraints are required
instead of the one given above, resulting here in the following program:

\indent $p \ASPor q.$\\
\indent $\leftarrow p, \ASPnot \K\ p.$\\
\indent $\leftarrow \leftASPnot \M\ p.$

\noindent
So with ES2014 semantics we now have a program with no world view. The same is
true in this case with the later ES2016 semantics; however, the new maximality
requirement in ES2016 means such ``tricks'' won't work for all programs.
Consider the following:

\indent $p \leftarrow \M\ q, \ASPnot q.$\\
\indent $q \leftarrow \M\ p, \ASPnot p.$\\
\indent $r \leftarrow \M\ p,~\M\ q.$

\noindent
Under ES2014 semantics, $\{\{\}\}$ and $\{\{p,r\},\{q,r\}\}$ are the world
views. Per ES2016, only the latter is a world view. If we now add the
constraint

\indent $\leftarrow \K\ r.$

\noindent
the resulting program has world view $\{\{\}\},$ which is not an ES2016 world
view without this constraint. We observe that there does not appear to be
a general way to simply rule out world views under ES2016 semantics.
This observation leads to our thesis.

{\bf As the semantics of Epistemic Specifications has evolved to address
unintended world views and support intuition with respect to certain programs,
we believe the added complexity has had a negative side effect with respect to
intuitive understanding of certain other programs---particularly those
involving constraints with subjective literals.} Thus, in an attempt to
facilitate correct problem encoding/program development in line with intuition,
we propose a new language construct called a \emph{world view constraint} (WVC)
and introduce symbol $\WVCarrow$ read as ``it is not a world view (if...)'' for
use in forming a WVC. For example,

\indent $\WVCarrow ~\K\ p.$

\noindent
is read ``it is not a world view if $p$ is known'' and
means (informally) that any world view satisfying ~$\K\hspace{0.07cm}p$~ is
ruled out from the set of world views of the program under consideration.
This is analogous to how constraints affect answer sets in ASP, though at the
world view level for Epistemic Specifications.

